Analysis and Optimization of Graph Decompositions by Lifted Multicuts

We study the set of all decompositions (clusterings) of a graph through its characterization as a set of lifted multicuts. This leads us to practically relevant insights related to the definition of a class of decompositions by must-join and must-cut constraints and related to the comparison of clusterings by metrics. To find optimal decompositions defined by minimum cost lifted multicuts, we establish some properties of some facets of lifted multicut polytopes, define efficient separation procedures and apply these in a branch-and-cut algorithm.

==> figures/cuts-examples.tex <==
\begin{subtikzpicture}{a)}
\draw[green] plot [smooth, tension=2] coordinates {(0, 0) (1, 0.7) (2, 0)};
\node[style=vertex,label=left:$v$] at (0, 0) (v) {};
\node[style=vertex] at (1, 0) (s) {};
\node[style=vertex,label=right:$w$] at (2, 0) (w) {};
\node[style=vertex] at (1.5, -0.75) (t) {};
\draw (v) -- (s);
\draw[style=cut-edge] (s) -- (w);
\draw[style=cut-edge] (s) -- (t);
\draw (t) -- (w);
\node at (1.5, 0.2) {$e'$};
\node at (1.1, -0.5) {$e$};
\node at (1, 0.9) {$\color{green}f$};
\end{subtikzpicture}
\hfill
\begin{subtikzpicture}{b)}
\draw (0, 0) -- (0.6, 0);
\draw[style=cut-edge] (0.6, 0) -- (1.3, 0);
\draw (2, 0) -- (1.3, 0);
\draw[green] plot [smooth, tension=2] coordinates {(0.6, 0) (1.3, -0.5) (2, 0)};
\draw[green] plot [smooth, tension=2] coordinates {(0, 0) (1, 0.7) (2, 0)};
\node[style=vertex] at (0, 0) (v) {};
\node[style=vertex] at (0.6, 0) (r) {};
\node[style=vertex] at (1.3, 0) (n2) {};
\node[style=vertex] at (2, 0) (w) {};
\node at (1.3, -0.8) {$\color{green}f'$};
\node at (1, 0.9) {$\color{green}f$};
\node[label=left:$v$] at (0, 0) {};
\node[label=above:$r$] at (0.6, 0) {};
\node[label=right:{$w=s$}] at (2, 0) {};
\end{subtikzpicture}
\hfill
\begin{subtikzpicture}{c)}
\draw[style=cut-edge] (0, 0) -- (1, 0);
\draw (0, 0) -- (0,-1);
\draw (1, 0) -- (1,-1);
\draw[style=cut-edge] (0,-1) -- (1,-1);
\draw[green] (0,-1) -- (1,0);
\draw[green] plot [smooth, tension=2] coordinates {(0, 0) (1.3, 0.3) (1,-1)};
\node[style=vertex] at (0, 0) {};
\node[style=vertex] at (1, 0) {};
\node[style=vertex] at (0,-1) {};
\node[style=vertex] at (1,-1) {};
\node at (0.5, 0.2) {$e$};
\node at (0.4, -0.4) {$\color{green}f'$};
\node at (0.9, 0.7) {$\color{green}f$};
\node at (0.5, -1.2) {$e'$};
\node[label=left:$v$] at (0, 0) {};
\node[label=left:{$r$}] at (0,-1) {};
\node[label=right:$s$] at (1, 0) {};
\node[label=right:{$w$}] at (1,-1) {};
\end{subtikzpicture}
\hfill
\begin{subtikzpicture}{d)}
\draw (0, 0) -- (1, 0);
\draw[style=cut-edge] (1, 0) -- (2, 0);
\draw[style=cut-edge] (1, -0.75) -- (2, 0);
\draw (2, 0) -- (3, 0);
\draw (0, 0) -- (1, -0.75);
\draw[green] plot [smooth, tension=2] coordinates {(0, 0) (1.5, 1) (3, 0)};
\draw[green] plot [smooth, tension=2] coordinates {(1, 0) (2, 0.7) (3, 0)};
\node[style=vertex] at (0, 0) {};
\node[style=vertex] at (1, 0) {};
\node[style=vertex] at (2, 0) {};
\node[style=vertex] at (3, 0) {};
\node[style=vertex] at (1, -0.75) {};
\node at (1.5, 0.2) {$e_0$};
\node at (1.75, -0.5) {$e_1$};
\node at (2, 0.5) {$\color{green}f'$};
\node at (1.5, 1.2) {$\color{green}f$};
\node[label=left:$v$] at (0, 0) {};
\node[label=right:{$w$}] at (3, 0) {};
\end{subtikzpicture}
\\
\begin{subtikzpicture}{e)}
\draw[green] plot [smooth, tension=2] coordinates {(0, -0.3) (3,-1.5) (0,-2.7)};
\node at (3.2,-1.5) {$\color{green}f$};
\node[style=vertex,label=above:{$v$}] (v) at (0,-0.3) {};
\node[style=vertex] (1) at (2.3,-1) {};
\node[style=vertex] (2) at (1.5,-1) {};
\node[style=vertex] (3) at (0.8,-1) {};
\node[style=vertex] (4) at (-0.8,-1) {};
\node[style=vertex] (5) at (-1.5,-1) {};
\node[style=vertex] (6) at (-2.3,-1) {};
\node[style=vertex] (7) at (2.3,-2) {};
\node[style=vertex] (8) at (1.5,-2) {};
\node[style=vertex] (9) at (0.8,-2) {};
\node[style=vertex] (10) at (-0.8,-2) {};
\node[style=vertex] (11) at (-1.5,-2) {};
\node[style=vertex] (12) at (-2.3,-2) {};
\node[style=vertex,label=below:{$w$}] (w) at (0,-2.7) {};
\draw[-] (v) edge [bend left=15] (1);
\draw[-] (v) edge [bend right=15] (6);
\draw[-] (w) edge [bend right=15] (7);
\draw[-] (w) edge [bend left=15] (12);
\draw[-] (1) edge (2);
\draw[-] (2) edge (3);
\draw[-] (3) edge (4);
\draw[-] (4) edge (5);
\draw[-] (5) edge (6);
\draw[-] (7) edge (8);
\draw[-] (8) edge (9);
\draw[-] (9) edge (10);
\draw[-] (10) edge (11);
\draw[-] (11) edge (12);
\draw[style=cut-edge] (1) edge (7);
\draw[style=cut-edge] (1) edge (8);
\draw[style=cut-edge] (2) edge (7);
\draw[style=cut-edge] (3) edge (9);
\draw[style=cut-edge] (4) edge (10);
\draw[style=cut-edge] (5) edge (12);
\draw[style=cut-edge] (6) edge (11);
\draw[style=cut-edge] (6) edge (12);
\draw[-,green] (3) edge node[above=10,right=-5] {$f_1$} (10);
\draw[-,green] (4) edge node[below=10,right=-5] {$f_2$} (9);
\end{subtikzpicture}
\hfill
\begin{subtikzpicture}{f)}
\draw (0, 0) -- (1, 0);
\draw[style=cut-edge] (2, 0) -- (1,0);
\draw (2, 0) -- (3, 0);
\draw[green] plot [smooth, tension=2] coordinates {(0, 0) (1.5, 1) (3, 0)};
\draw[green] plot [smooth, tension=2] coordinates {(1, 0) (2, 0.5) (3, 0)};
\draw[green] plot [smooth, tension=2] coordinates {(0, 0) (1, -0.5) (2, 0)};
\node[style=vertex] at (0, 0) {};
\node[style=vertex] at (1, 0) {};
\node[style=vertex] at (2, 0) {};
\node[style=vertex] at (3, 0) {};
\node at (1.5, 1.2) {$\color{green}f'$};
\node at (2, 0.7) {$\color{green}f''$};
\node at (1, -0.7) {$\color{green}f$};
\node[label=left:{$v$}] at (0, 0) {};
\node[label=below:$w$] at (2.2, 0) {};
\end{subtikzpicture}
%\end{comment}
\hfill
\begin{subtikzpicture}{g)}
\draw[green] plot [smooth, tension=2] coordinates {(0, 0) (1.3, 1) (2.6, 0)};
\node at (1.3, 1.25) {$\color{green}f'$};
\node[style=vertex] (1) at (0, 0) {};
\node[style=vertex,label=below:$v$] (2) at (0.7, 0) {};
\node[style=vertex] (3) at (1.4, 0) {};
\node[style=vertex] (4) at (2, 0.6) {};
\node[style=vertex] (5) at (2, -0.6) {};
\node[style=vertex,label=below:$w$] (6) at (2.6, 0) {};
\draw (1) -- (2);
\draw (2) -- (3);
\draw[style=cut-edge] (3) -- (4);
\draw[style=cut-edge] (3) -- (5);
\draw (4) -- (6);
\draw (5) -- (6);
\draw[-,green] (1) edge [bend left=18] node[above] {$f_1$} (4);
\draw[-,green] (1) edge [bend right=18] node[below] {$f_2$} (5);
\draw[-,green] (2) edge [bend left=33] node[below=8,right=0] {$f$} (6);
\end{subtikzpicture}
\\
\begin{subtikzpicture}{h)}
\draw (0.5, 0) -- (1, 0);
\draw (1, 0) -- (1.5, 0.5);
\draw (1.5, 0.5) -- (2, 1);
\draw[style=cut-edge] (2, 1) -- (2.5, 1);
\draw (2.5, 1) -- (3.5, 0);
\draw (1, 0) -- (2, -1);
\draw[style=cut-edge] (2, -1) -- (2.5, -1);
\draw (2.5, -1) -- (3, -0.5);
\draw (3, -0.5) -- (3.5, 0);
\draw (3.5, 0) -- (4, 0);
\draw[green] plot coordinates {(1.5, 0.5) (3.5, 0)};
\draw[green] plot coordinates {(1.5, 0.5) (3, -0.5)};
\draw[green] plot coordinates {(1, 0) (3, -0.5)};
\draw[green] plot [smooth, tension=2] coordinates {(0.5, 0) (2.25, 1.25) (4, 0)};
\node[style=vertex] at (0.5, 0) {};
\node[style=vertex] at (1, 0) {};
\node[style=vertex] at (1.5, 0.5) {};
\node[style=vertex] at (2, 1) {};
\node[style=vertex] at (2.5, 1) {};
\node[style=vertex] at (2, -1) {};
\node[style=vertex] at (2.5, -1) {};
\node[style=vertex] at (3, -0.5) {};
\node[style=vertex] at (3.5, 0) {};
\node[style=vertex] at (4, 0) {};
\node at (2.5, 0.45) {$\color{green}f_3$};
\node at (2.7, 0) {$\color{green}f_2$};
\node at (2, -0.45) {$\color{green}f_1$};
\node at (2.25, 1.45) {$\color{green}f$};
\node[label=left:{$v$}] at (0.5, 0) {};
\node[label=above:{$v'$}] at (1, 0) {};
\node[label=above:{$w'$}] at (3.5, 0) {};
\node[label=right:{$w$}] at (4, 0) {};
\end{subtikzpicture}
\hfill
\begin{subtikzpicture}{i)}
\draw[green] plot [smooth, tension=2] coordinates {(0, 1.1) (1.4, 1.1) (1.1, -1.1)};
\node at (1.5,1.3) {$\color{green}f$};
\node[style=vertex,label=left:{$v=v'$}] (v) at (0,1.1) {};
\node[style=vertex] (1) at (0,0) {};
\node[style=vertex] (2) at (0,-1.1) {};
\node[style=vertex] (3) at (1.1,1.1) {};
\node[style=vertex] (4) at (1.1,0) {};
\node[style=vertex,label=right:{$w=w'$}] (w) at (1.1,-1.1) {};
\draw[-,green] (1) edge node[above=2,left=1] {$f_1$} (3);
\draw[-,green] (1) edge node[above=2,right=1] {$f_2$} (w);
\draw[-,green] (1) edge node[above=8,right=1] {$f'$} (4);
\draw[-] (v) edge (1);
\draw[-] (1) edge (2);
\draw[-] (3) edge (4);
\draw[-] (4) edge (w);
\draw[style=cut-edge] (v) edge node[above] {$e$} (3);
\draw[style=cut-edge] (2) edge (w);
\end{subtikzpicture}
\hfill
\begin{subtikzpicture}{j)}
\draw (0.5, 0) -- (1, 0);
\draw (1, 0) -- (1.5, 0.5);
\draw (1.5, 0.5) -- (2, 1);
\draw (2, 1) -- (2.5, 1);
\draw[style=cut-edge] (2.5, 1) -- (3, 1);
\draw (3, 1) -- (4.5, 0);
\draw (4.5, 0) -- (5, 0);
\draw (1, 0) -- (2.5, -1);
\draw[style=cut-edge] (2.5, -1) -- (3, -1);
\draw (3, -1) -- (3.5, -1);
\draw (3.5, -1) -- (4, -0.5);
\draw (4, -0.5) -- (4.5, 0);
\draw[green] (1.5, 0.5) -- (3.5, -1);
\draw[green] (1.5, 0.5) -- (4, -0.5);
\draw[green] (2, 1) -- (3.5, -1);
\draw[green] (2, 1) -- (4, -0.5);
%\draw[green] plot coordinates {(1.5, 0.5) (3.5, 0)};
%\draw[green] plot coordinates {(1.5, 0.5) (3, -0.5)};
%\draw[green] plot coordinates {(1, 0) (3, -0.5)};
\draw[green] plot [smooth, tension=2] coordinates {(0.5, 0) (2.75, 1.25) (5, 0)};
\node[style=vertex] at (0.5, 0) {};
\node[style=vertex] at (1, 0) {};
\node[style=vertex] at (1.5, 0.5) {};
\node[style=vertex] at (2, 1) {};
\node[style=vertex] at (2.5, 1) {};
\node[style=vertex] at (3, 1) {};
\node[style=vertex] at (4.5, 0) {};
\node[style=vertex] at (5, 0) {};
\node[style=vertex] at (2.5, -1) {};
\node[style=vertex] at (3, -1) {};
\node[style=vertex] at (3.5, -1) {};
\node[style=vertex] at (4, -0.5) {};
\node at (2.75, 1.45) {$\color{green}f$};
\node at (3.1, 0.5) {$\color{green}f_1$};
\node at (2.1, 0.6) {$\color{green}f_2$};
\node at (2.5, -0.5) {$\color{green}f_3$};
\node at (3.5, -0.5) {$\color{green}f_4$};
\node[label=below:{$v$}] at (0.5, 0) {};
\node[label=below:{$w$}] at (5, 0) {};
\end{subtikzpicture}
\hfill
\begin{subtikzpicture}{k)}
\draw[green] plot [smooth, tension=2] coordinates {(0, 1.3) (1.6, 1.3) (1.3, -1.1)};
\node at (1.7,1.5) {$\color{green}f$};
\node[style=vertex,label=left:{$v$}] (v) at (0,1.3) {};
\node[style=vertex] (1) at (0,0) {};
\node[style=vertex] (2) at (0,-1.1) {};
\node[style=vertex] (3) at (1.3,1.3) {};
\node[style=vertex] (4) at (1.3,0) {};
\node[style=vertex,label=right:{$w$}] (w) at (1.3,-1.1) {};
\draw[-,green] (v) edge node[above=5,left=6] {$f_3$} (4);
\draw[-,green] (1) edge node[above=5,right=6] {$f_1$} (3);
\draw[-,green] (1) edge node[below] {$f_2$} (4);
\draw[-] (v) edge (1);
\draw[-] (1) edge (2);
\draw[-] (3) edge (4);
\draw[-] (4) edge (w);
\draw[style=cut-edge] (v) edge node[above] {$e$} (3);
\draw[style=cut-edge] (2) edge (w);
\end{subtikzpicture}


==> figures/dimension-example.tex <==
\mbox{%
\begin{subtikzpicture}{a)}
\draw (0, 0) to (3, 0);
\draw[green] plot [smooth, tension=2] coordinates {(0, 0) (1, 0.7) (2, 0)};
\draw[green] plot [smooth, tension=2] coordinates {(1, 0) (2, 0.7) (3, 0)};
\draw[green] plot [smooth, tension=2] coordinates {(0, 0) (1.5, 1.3) (3, 0)};
\node[rectangle, draw=none, fill=none] at (1, 0.9) {$\color{green}f_1$};
\node[rectangle, draw=none, fill=none] at (2, 0.9) {$\color{green}f_2$};
\node[rectangle, draw=none, fill=none] at (1.5, 1.5) {$\color{green}f_3$};
\node[style=vertex, label=below:$v_1$] at (0, 0) {};
\node[style=vertex, label=below:$v_2$] at (1, 0) {};
\node[style=vertex, label=below:$v_3$] at (2, 0) {};
\node[style=vertex, label=below:$v_4$] at (3, 0) {};
\end{subtikzpicture}
\hfill
\begin{subtikzpicture}{b)}
\draw (0.8, 1.6) to (0, 0.8) to (0.8, 0) to (1.8, 0) to (2.6, 0.8) to (1.8, 1.6) to (0.8, 1.6);
\draw[green] (0.8, 0) to (1.8, 1.6);
\draw[green] (0.8, 0) to (0.8, 1.6);
\draw[green] (1.8, 0) to (1.8, 1.6);
\node[style=vertex, label=left:$v_2$] at (0, 0.8) {};
\node[style=vertex, label=below:$v_3$] at (0.8, 0) {};
\node[style=vertex, label=below:$v_4$] at (1.8, 0) {};
\node[style=vertex, label=right:$v_5$] at (2.6, 0.8) {};
\node[style=vertex, label=above:$v_6$] at (1.8, 1.6) {};
\node[style=vertex, label=above:$v_1$] at (0.8, 1.6) {};
\node[rectangle, draw=none, fill=none] at (0.6, 0.8) {$\color{green}f_1$};
\node[rectangle, draw=none, fill=none] at (2, 0.8) {$\color{green}f_2$};
\node[rectangle, draw=none, fill=none] at (1.1, 0.8) {$\color{green}f_3$};
\end{subtikzpicture}}

